STASH: Securing transparent authentication schemes using prover-side proximity verification

Transparent authentication (TA) schemes are those in which a user is authenticated by a verifier without requiring explicit user interaction. By doing so, those schemes promise high usability and security simultaneously. The majority of TA implementations rely on the received signal strength as an indicator for the proximity of a user device (prover). However, such implicit proximity verification is not secure against an adversary who can relay messages over a larger distance. In this paper, we propose a novel approach for thwarting relay attacks in TA schemes: the prover permits access to authentication credentials only if it can confirm that it is near the verifier. We present STASH, a system for relay-resilient transparent authentication in which the prover does proximity verification by comparing its approach trajectory towards the intended verifier with known authorized reference trajectories. Trajectories are measured using low-cost sensors commonly available on personal devices. We demonstrate the security of STASH against a class of adversaries and its ease-of-use by analyzing empirical data, collected using a STASH prototype. STASH is efficient and can be easily integrated to complement existing TA schemes.

==> Makefile <==
# Check  style:
MAINFILE = main
FILES = 0_introduction 1_assumptionsandgoals 2_systemprototype 3_experimentalevaluation 5_securityanalysis 6_discussion 7_relatedwork 8_conclusion main
build:
	pdflatex $(MAINFILE).tex
	bibtex $(MAINFILE)
	pdflatex $(MAINFILE).tex
	pdflatex $(MAINFILE).tex

submission:
	pdflatex submission.tex
	bibtex submission
	pdflatex submission.tex
	pdflatex submission.tex

# Use '- ' before a command to tell Make to continue running even if output is non-zero
proof:
	echo "weasel words: "
	- bash ~/work/pers/utils/bin/weasel.sh $(MAINFILE).tex
	echo
	echo "passive voice: "
	- bash ~/work/pers/utils/bin/passive.sh $(MAINFILE).tex
	echo
	echo "duplicates: "
	- perl ~/work/pers/utils/bin/duplicates.pl $(MAINFILE).tex
	echo
	echo "Detect improper citations or refs (wrong spaces, no spaces, etc.)"
	- grep -E '[^~]\\cite' $(MAINFILE).tex --color
	- grep -E '[^~]\\ref' $(MAINFILE).tex --color
	- grep -E 'on Figure' $(MAINFILE).tex --color
	- grep -E 'TODO' $(MAINFILE).tex --color

# Ensure that no links are left in the bibtex file
	- grep -E '(url|URL)\s*=' *.bib --color

	echo "Do you need to run a spellchecker as well?"

# TODO: ideja: napravit file koji detektira inconsistencies kod koristenja nekih rijeci, npr, -ize/-ise, non-linear/nonlinear itd


# Spell Checker
spelling:
	@$(foreach file,$(FILES),aspell --lang=en_US --mode=tex check $(file).tex;)

clean:
	~/work/pers/utils/cleanAll.sh

